"AI enhances our performance, I have no doubt this one will do the same": The Placebo effect is robust to negative descriptions of AI

Heightened AI expectations facilitate performance in human-AI interactions through placebo effects. While lowering expectations to control for placebo effects is advisable, overly negative expectations could induce nocebo effects. In a letter discrimination task, we informed participants that an AI would either increase or decrease their performance by adapting the interface, but in reality, no AI was present in any condition. A Bayesian analysis showed that participants had high expectations and performed descriptively better irrespective of the AI description when a sham-AI was present. Using cognitive modeling, we could trace this advantage back to participants gathering more information. A replication study verified that negative AI descriptions do not alter expectations, suggesting that performance expectations with AI are biased and robust to negative verbal descriptions. We discuss the impact of user expectations on AI interactions and evaluation and provide a behavioral placebo marker for human-AI interaction

==> misc/old_text.tex <==
%


%\todo{What is the specific problem addressed?}




%\mychange{~\cite{finniss2010biological,powerless2001}} without treating the patient with an active substance or specific procedure. Such a placebo can alleviate pain~\cite{lasagna1954study} or support the treatment of ailments~\cite{beecher1955powerful, kaptchuk1998powerful}, thereby providing an effective medical treatment without an illness-specific mechanism of effect. The only critical determinant of the placebo effect is the patient's expectation in the placebo's efficacy, \mychange{leading to a positive evaluation after treatment~\cite{stewart2004placebo, montgomery1996mechanisms}}. 


% \todo{What have you done?}
% \todo{What did you find out?}
% \todo{What are the implications on a larger scale?}
% Placebo, as induced by heightened expectations in technology interaction, can obscure evaluation.  In this study, we investigate whether expectations can be manipulated to show a nocebo effect in an AI user study.
% We examined the influence of a negative description of an AI system on rapid interactive decision-making task. Participants were led to believe that an adaptive AI system would decrease (nocebo) their task performance when in fact, no AI system was active. Participants did not believe in the decrease of their performance. Using cognitive modeling, we could identify that in the nocebo condition, participants exhibited a more conservative decision criterion as compared to the control condition. We also replicate the placebo effect of AI systems. We discuss the implications of negative expectations on Human-AI interaction and show that cognitive modeling might be able to detect placebo/nocebo response in AI-augmented decision-making.

%Society harbors hopes and fears with regard to AI. Heightened expectations in AI can affect Human-AI interaction in the form of placebo effects. In a letter identification task, we informed participants that an AI system would either positively or adversely affect their performance, though no AI was operational. The results showed that irrespective of the description, participants under this AI sham condition, had high expectations concerning performance gains and were faster while not changing their accuracy. Cognitive modeling with a Wiener Drift-Diffusion process, could show that participants attained information with a sham AI faster compared to a control condition. Additionally, our second study successfully replicated the lack of an effect of negative description on expectation. We add to the literature on placebo effects of AI the first study showing a main effect on performance indicators, a marker that can be obtained via a computational model of decision making and a robustness check with regard to negative verbal descriptions of the AI system. We highlight the profound influence of user expectations on AI interactions and advocate for the potential of cognitive modeling to discern placebo reactions in AI-supported decision-making processes.
%Recent~\cite{villa} research indicated that introducing a sham AI-augmentation technology to usaers, a placebo treatment inducing the expectation of improved performance, can lead to riskier decision-making. Thus, expectations seem to shape how interaction with AI systems unfolds and how we make decisions. %In this paper, we will use cognitive modeling to demonstrate how decision-making is affected by positive (placebo) and negative expectations (nocebo) and discuss how nocebo effects may hinder optimal Human-AI interaction. 
 %These hopes and concerns could influence Human-AI interaction, leading to a potential effect where expectations about the AI system's performance affect individual outcomes of a user study.  %and thus negative expectations may likewise affect Human-AI interaction. % go on about concerns
% A nocebo effect in Human-AI interaction will manifest in a user study if a user's negative expectations about Human-AI performance affect individual study outcomes.
% Second Paragraph
% CORE MESSAGE OF THIS PARAGRAPH:
%\todo{P2. The second paragraph should be about what have others been doing}

% We examined the influence of a negative verbal description to elicit a nocebo response, and positive verbal descriptions (placebo) on decision-making in a letter identification task when using a sham adaptive AI system. Counter to our initial goal of the study of investigating a nocebo effect, \footnote{We pre-registered the experimental study here and deviated substantially from the study plan due to a lack of a nocebo response.} an induction of negative expectations via verbal descriptions was not possible. From two subsequent studies articipants' expectations with regard to their joint performance with an adaptive AI system were robustly positive, resembling \citet{kosch2022placebo,villa2023placebo} and could only be set to a neutral but never truly negative expectancy. 

 
 % We then analyzed the behavioral data and could find reaction times to be faster when subjected to the AI condition as compared to the control condition. Cognitive modelling, with the drift-diffusion model, revealed that in the AI condition participants gathered information faster as compared to the control condition.  This is mirrored in the subjective feedback of participants regarding the usability of the system, user experience and the ease of the task. We did not find any effect of our manipulations on workload subjective or physiological indicators of workload (EDA). Considering the grave implications of our inability to induce negative expectations with regard to an AI system, a no-nocebo effect of AI, we ran two online replication studies (n=50 each). In both studies, participants believed that they would perform better with an AI system, although they were explicitly told their performance would get worse as compared to no-AI support. 




%\todo{P3.5. What is new about your work?}
%We add to the literature on placebo effects in HCI a study that shows how negative expectations concerning AI can hinder optimal decision-making in human-machine interaction. 
% Fourth paragraph
% CORE MESSAGE OF THIS PARAGRAPH:
%\todo{P4.6. What did you find out? What are the concrete results?}
% \textcolor{red}{ Used cognitive modeling, and drift-diffusion modeling. We found that while for neutral expectations, decision-making was unaffected by our sham manipulation, positive expectations with regard to a sham AI system directly influence decision-making, Participants decision criterion was more liberal and responses were faster as indicated by a  smaller decision boundary while the accumulation of information for participants (drift rate) was unaffected. This is mirrored in the subjective feedback of participants regarding the usability of the system and a relatively increased physiological arousal as measured by electrodermal activity (EDA), a proxy for participants' cognitive workload. There were no differences for neutral expectations but a decreased feeling of workload, reduced EDA and better subjective usability for the placebo-condition. }
 
 
 % to reveal that negative expectations make decision-making with adaptive AI systems more conservative (decision boundary), leading to fewer errors but much-prolonged reaction times while not changing the accumulation of information in participants (drift rate). This is mirrored in the subjective feedback of participants regarding the usability of the system and a relatively increased physiological arousal as measured by electrodermal activity (EDA), a proxy for participants' cognitive workload. We replicate previous studies \cite{Kosch} by showing the reverse pattern of effects in a placebo group. 
%\todo{P4.7. What are the implications? What does this mean for the bigger picture?}


% Our results resonate with recent calls in HCI to control and/or measure expectations in evaluating intelligent systems. We add to this a cautionary note that positive expectations about Human-AI performance are much easier to implement than negative expectations. On a behavioral level, we provide a behavioral marker for the placebo response, a change in the decision boundary, that can be implemented in intelligent systems for research and application purposes. %On a subjective level, participants report interaction to be more cumbersome and on a physiological level, physiological arousal can increase. W
% e follow that in a human-centered design process, evaluation in HCI must be regarded as a function of user expectation and that AI narratives will make it challenging to level out expectations.  
% %In placebo-controlled pharmacological studies, participants with impairments are unaware whether they were administered an active (e.g., painkiller) or inactive treatment (e.g., a sugar pill). Therefore, in evaluating these studies, a treatment is considered successful only if its effect supersedes the placebo effect.
% In a user-centered design process, systems are probed by a user, typically by comparing  interaction with a standard technology to new technology. In these studies, users can often discern the experimental conditions, e.g., a new AI system vs. a baseline system. 
% Instructions may even indicate the novelty of the tested systems~\cite{21Waystonudge} explicitly. Therefore, studies in technology evaluation can set expectations a-priori that may evaluation of systems (for a more nuanced discussion on expectations, see e.g., \cite{kujala2017role}). While positive expectations (placebo) have been shown to improve study outcomes \cite{kosch2022placebo} leading to overconfidence in the researcher regarding the attributes of the system (usability or user experience), negative expectations could harm user-centered design by leading designers to make changes to the system that are unnecessary or even detrimental to Human-AI performance.
%
%Nocebo effects much like placebo effects undermine evaluation in studies with human subjects
%Nocebo effects could hinder technology adoption
%
%hus, while the placebo effect is well-established work that shows how to mitigate placebo effects and investigate the whole spectrum of expectations, including negative expectations, is scarce.  
% - Little known about large scale effects of AI adoption
% - EVALUATION
% - 
%
%Much like placebo effects, the nocebo effect can obscure the evaluation of medical interventions. 


%RW


% Note that while previous research has looked at people's expectations with regard to transparency \cite{meurisch_exploring_2020,park_human-ai_2021,purcell_fears_2023}, the Human-ai relation \cite{zhang_ideal_2021} or autonomy \cite{meurisch_exploring_2020} to inform the design of AI interfaces, scientific knowledge is scarce with respect to outcome expectations (e.g., how people think they will perform with a system\cite{kosch2022placebo}). 


% People's pre-existing attitudes and experiences with AI systems also can impact their acceptance of AI in collaborative tasks. A study researched how individuals perceive AI teammates and their expectations in multiplayer online games. Based on the results, individuals generally have a favorable view of collaborating with AI teammates. The study identifies expectations such as instrumental skills, shared understanding, communication abilities, human-like behaviors, and performance \cite{zhang_ideal_2021}.



% Therefore, expectations around AI in the general population tend to be more negative than positive.

% Another factor that influences the perception of AI is system transparency \cite{meurisch_exploring_2020,park_human-ai_2021,purcell_fears_2023}. This has been found when investigating AI-mediated communication technologies \cite{purcell_fears_2023} and implementing AI systems in human resource management \cite{park_human-ai_2021}. Individuals are more likely to object if the use of AI is not disclosed and tend to expect others to use AIs more than they themselves would. Interestingly, individuals appear to be more at ease with the idea of others using AI assistants than using them personally. However, the study also found that individuals tend to have negative expectations of AI due to concerns that others may use them irresponsibly \cite{purcell_fears_2023}. Hence, it is crucial to consider transparency while designing new AI products.

% Additionally, the perception and ultimately the acceptance of AI systems also depend on the system's level of autonomy. Individuals who prefer less proactive systems are concerned about privacy and mistrust the AI, while those who prefer more proactivity have optimistic expectations and believe the AI can enhance their quality of life \cite{meurisch_exploring_2020}.

% \todo{maybe take out or just mention multiplayer games} People's pre-existing attitudes and experiences with AI systems also can impact their acceptance of AI in collaborative tasks. A study researched how individuals perceive AI teammates and their expectations in multiplayer online games. Based on the results, individuals generally have a favorable view of collaborating with AI teammates. The study identifies expectations such as instrumental skills, shared understanding, communication abilities, human-like behaviors, and performance \cite{zhang_ideal_2021}.


% Initially, AI was used to improve the quality of data, particularly in complex areas such as healthcare and logistics. Research conducted by \citet{beede2020human} and \citet{min2021} has demonstrated the effectiveness of AI in detecting eye diseases and aiding clinical decision-making, respectively. Additionally, \citet{abidi2006improving} showed how AI-based pseudocoloring of objects in luggage x-rays can significantly enhance operational performance. However, AI-based decision support systems, similar to human-automation systems, can lead to more liberal or conservative decision-making \cite{ingrams2022ai}. Automation bias is a well-known phenomenon, which describes a more liberal decision-making when relying on automated systems\cite{skitka1999does}. This bias is present in both novices and experts \cite{parasuraman2010complacency}, and is only partially mitigated by trust-calibration or AI explanations \cite{zhang2020effect}, suggesting the need for a rethinking of trust towards responsivity and resilience in Human-AI interaction \cite{chiou2023trusting}. Therefore, while AI increases performance by providing more information and improving access to it, it can also introduce biases such as automation bias.

%\todo{add some juice to nocebo studies}
 %Numerous studies have demonstrated that the placebo effect can improve a condition, promote creativity, improve cognitive ability, and boost athletic performance \cite{Beedie2019Incorporating, Oken2007Expectancy, BEEDIE2006Placebo, weger2013rapid, rozenkrantz2017placebo, WATKINS198671, BELCHIOR20131318}. This indicates that a placebo affects the individual's state.
%Irrespective of the measurement outcome, the subject's mental model of the effect of treatment is crucial for the placebo effect to manifest. Previous research has shown that expectancy can not only be induced regarding the outcome (response expectancy) ~\cite{kirsch1999specifying,Oken2007Expectancy, lee2020expectancy}, biasing the participant's perception of their reaction (e.g., the placebo alleviating the feeling of pain), but also that evaluation of the stimulus itself can be biased (stimulus expectancy), e.g., the placebo reducing the perception of pain. Implementing response expectancies is the more dominant and robust paradigm ~\cite{kirsch1999specifying} for eliciting placebo effects; therefore, our sham augmentation will, therefore, focus on the implementation of response expectancies. 


% \subsection{Adaptive interfaces}
%  The adaptation of UIs has become an integral part of interactive systems to satisfy the user's goals, widen the user base, and extend the system's lifespan~\cite{browne2016adaptive}. User-centric adaptation can span from the content or the interface format and the different user input modalities. For example, one can adapt letter presentation in an E-reader to alpha oscillations, an indicator of workload in the electroencephalogram \cite{koschrsvp}, reduce the number of interaction possibilities with the number of errors made by the user \cite{hudlicka2002assessment} or adapt the interface to the mood of the user \cite{10.1145/2668056.2668058}. Further examples include the user's context~\cite{10.1145/1216295.1216357} and their interaction performance as well as their physiology~\cite{10.1145/2808228} serving as implicit measurements for user interface adaptations. Many user interfaces base their adaptations on AI-methods. The availability of large-scale user data allowed recent advances in machine learning and neural networks to make robust predictions about user-related issues during interaction. This includes adaptations based on the user's perceived workload~\cite{koschrsvp, 10.1145/3173574.3174010,      kosch2019your}, emotions~\cite{10.1145/3472749.3474775, 10.1145/3399715.3399928},       and interaction difficulties due to the complex visualization of UI elements~\cite{10.1145/3229093}.
 
%  AI-based adaptive interfaces optimize usability by linking the system design to user input~\cite{HORNBAEK200679}, where the overall goal of user interface adaptations is the improvement of the interaction efficiency and perceived usability~\cite{HORNBAEK200679}. However, previous placebo research~\cite{Duarte12, strait2014reliability, vaccaro2018illusion, Paepcke2010,kosch2022placebo} indicated that the sole description of a non-functional adaptive system can positively increase user satisfaction without system functionality. Therefore, descriptions of systems can be regarded as a potential placebo, if aside from perceived effectiveness task performance is susceptible to such manipulations \cite{Duarte12, 10.1145/1133265.1133306}    . 

 
 %While AI adaptive interfaces may change the decision boundary. This aligns with %
 
 %Furthermore, AI can personalize a user interface by learning from a user's patterns and preferences to increase usability and provide a better user experience. % add some physiology here

% AI has thus been used in various ways to augment human decision-making, from providing additional information to interface adaptations that streamline the task at hand. 




%This can be partly attributed to the paradox of experimental control in HCI. In medical trials, placebo effects are controlled by giving a non-active treatment to participants. Here, participants will not know whether they have been given the active treatment (e.g., a painkiller) or an inactive substance (e.g., a sugar pill). In HCI, participants often recognize the system or technique and can tell apart the experimental conditions, e.g., a novel AI system against a baseline system. Instructions by the experimenter might even explicitly describe the novelty of the evaluated systems and, hence, set participants' expectations and, therefore, produce a placebo effect. 

%For most AI technologies, it is challenging or nearly impossible to assess the functionality of the system because their underlying AI algorithms are complex, nonlinear and nontraceable. In line with this, previous studies have found that participants do not probe the functionality of AI systems~\cite{kosch2022placebo}. Therefore, users may assume a functional system producing a placebo effect of AI systems.




%We anticipated that a description of an AI in placebo affects the participant's decision-making. %Note that while trust and over-reliance are relevant to AI and their adoption, our study focused on the expectation of impairment and the nocebo effect's mechanism altering decision-making.


% Previous research has shown that social learning \citep{kirsch1999specifying}, classical conditioning \citep{flaten1999caffeine}, or verbal information (e.g., expert instructions \citep{stewart2004placebo}) can all be used to generate placebos. We concentrated on the latter and attempted to create a placebo effect by changing system descriptions \citep{kosch2022placebo}. We conducted a within-subjects lab study following medical research on the placebo effect \citep{gniss2020placebo} and HCI research on placebo effects \citep{kosch2022placebo} to determine the effect of expecting augmentation on risk-taking behavior. 
% %to answer the research question.  as a measure of risk-taking, 
% We operationalized risk-taking through the Columbia Card Task (CCT), the participants were given a revised version of the Hot CCT  two times, one per condition. In the augmentation condition, participants were told to be supported by a cognitive augmentation. In the no-augmentation condition, participants were told the augmentation system was turned off and that any beneficial effects did not exist. We anticipated that being cognitively augmented affected the participant's risk-taking behavior during the CCT. Note that while trust and over-reliance are relevant to ATs and their adoption, our study focused on the expectation of improvement and the placebo effect's mechanism altering risk-taking. %We conducted a within-subjects design following medical research on the placebo effect \citep{gniss2020placebo} and HCI research on placebo effects \citep{kosch2022placebo}.

% We used an EEG as a placebo AT and informed participants that the EEG was a Brain-Computer Interface (BCI) playing an inaudible sound that was proven to improve the ability to process information and thus perform better in the CCT. However, the setup was identical for both conditions, the system was not functional, and no sound was played. Note that our study was designed to show the placebo effect of an AT and that we did not focus on BCIs or the efficacy of augmentation of cognitive capacities per se, only on the propensity of placebo effects of ATs to increase risk-taking. 

% We adapted one aspect of the CCT for our study. Typically, in each round of the CCT, a participant is presented with a set of cards face down. Behind these are loss or win cards representing the given amount the player can win or lose. For the purpose of our study, participants were briefly presented with the cards face-up. Afterward, the cards were put face down again and shuffled using an animation. Participants were led to believe by the verbal description that the augmentation would support them in tracking the cards on the screen. Participants did not know that win or loss cards were rendered at each draw and that the whole game was rigged. 

% Note that medical research on pain-alleviating placebos has varied a large set of contextual variables that can modulate the placebo effect in size. \citet{wager2015neuroscience} provides a taxonomy of different contextual cues affecting placebo effects. These cues include the treatment cues (e.g., the novelty of the treatment), the place (e.g., a medical lab), the social situation (e.g., the experimenter wearing a white coat) and verbal suggestion (e.g., describing the mechanism closely); while we have taken these contextual variables into account, our study should resemble a user study for ATs as closely as possible. 

% To reiterate, we state the following research question:
% \begin{enumerate}
%     \item [\textbf{RQ}:] Can anticipation of being augmented be induced by verbal description and can this increase risk-taking behavior?
% \end{enumerate}
% We investigated the following hypotheses to answer this research question:
% \begin{enumerate}
% \item [\textbf{H1}:] A verbal description of an AT results in an increase in performance expections
% \item [\textbf{H2}:] A verbal description of an AT results in an increase in performance judgments after interaction
% \item [\textbf{H3}:] Performance expectations improvement induced by a placebo-treatment increases risk-taking behavior.
% \item [\textbf{H4}:] Performance expectations induced by a placebo-treatment affect processing of risk-related information.
% \end{enumerate}

%Additionally, they were provided with details about the system's status prior to commencing the letter discrimination task.
%\todo{(see~\autoref{fig:diagram1})}

%  \begin{figure}
%      \centering
%      \includegraphics[width=0.5\textwidth]{Content/Placebo Diag.pdf}
%      \caption{Stimulus: Verbal description; we told participants the EEG was a BCI system that modulated an inaudible sound that improves their information processing and RCCT performance. In reality, the system played no sound and was used to record data only.}
%      \label{fig:diagram1}
%  \end{figure}

% \begin{figure}[tbh]
%     \centering
%     \includegraphics[width=\textwidth]{Content/DiagramProcedure.pdf}
%     \caption{\ColorPrint Study flow diagram: We conducted a within-subjects study. We induced a placebo effect by changing system descriptions. Participants took the Revised Hot Columbia Card Task (RCCT) twice to measure risk-taking. Participants in the \textsc{augmentation} condition were told that they would be helped by a cognitive augmentation. In the \textsc{no-augmentation} condition, participants were told the augmentation system was off and no benefits existed. Finally, we informed them about the actual purpose of the study.}
%     \label{fig:diagram2}
% \end{figure}

from placeins package. prevents floats from passing a certain point.
%see \ref{fig:study_procedure}

%Risk-taking study - Study flow diagram: We conducted a within-subjects study. We induced a placebo effect by changing system descriptions. Participants took the Revised Hot Columbia Card Task (RCCT) twice to measure risk-taking. Participants in the augmentation condition were told that they would be helped by a cognitive augmentation. In the no-augmentation condition, participants were told the augmentation system was off and no benefits existed. Finally, we informed them about the actual purpose of the study.

%Additionally, they were informed that their response time and percentage of accurate responses would be analyzed.


% \begin{figure}[tbh]
%     \centering
%     \includegraphics[width=0.8\textwidth]{Content/Interface.png}
%     \caption{\ColorPrint RCCT interface: The interface was a deck of cards with five indicators: current round, number of points, loss and win card values, and number of loss cards. The interface permits players to skip and stop rounds.}
%     \label{fig:interface}
% \end{figure}


% Prior to starting the calibration, they were instructed to ask for the experimenter, who then provided the following verbal instructions:
% \begin{quote}
%     \textit{We will calibrate the baseline for the AI system now. It will record your physiological stress response and reaction times and adjust the pace of the task. Please use your index and middle finger to press the left and right arrow and respond to every letter you see, even if you are unsure. On the next screen you will be able to read all the instructions. Make sure you understand before continuing.}
% \end{quote}f
% The screen then displayed information stating that the calibration will personalize the AI system to their response behavior and stress level. 



%\begin{figure}
    %\centering
    %\includegraphics[width = 15.2cm]{instruction_figure.png}
    %\caption{Screen through a trial \agnes{TEST FIGURE, TO BE REPLACED}}
    %\label{fig:instruction_figure}
%\end{figure}
%see \ref{fig:instruction_figure}


% \paragraph{Sham calibration block}
% Participants also completed a practice block with 50 trials (using the comparison letters W/V) at the beginning of the experiment. This practice block was disguised as a calibration block, in which the participants were told that the AI system would be calibrated to their response behavior. Before the calibration block the text \textsc{Begin System Calibration} was shown for 7s. After the block, the text \textsc{Saving System Calibration} was displayed for 10s. To later reference the calibration block and to make the system more believable, a text stating that the AI system calibration was being retrieved was shown for 20s before the sham AI condition. For the no-AI condition, the text instead read \textsc{Preparing task}. Only after the sham AI condition, an additional window stating \textsc{Deactivating System} was shown for 5s.

%\todo{Table with results: The following nine questions were asked: \textit{I performed better in the task with the AI system than in the task without it (1), The task was easy (2), The AI system made the task easier (3), The AI system made the task more enjoyable (4), The AI system made me more self-confident (5), The AI system made me more efficient (6), The AI system improved my performance (7), The AI system improved my cognitive abilities (8), The AI system has a lot of potential for future development (9).}}


% \paragraph{Subjective Information Processing Awareness Scale}
% The Subjective Information Processing Awareness Scale (SIPAS) is a questionnaire that assesses how users perceive, understand, and predict information processing when interacting with intelligent systems \cite{Schrills_Franke_2021_SIPAS}. Originally consisting of 12 items \cite{Schrills_2021_SIPAS_validation}, it has since been validated and shortened to 6 items \cite{ Schrills_Franke_2023_SIPAS_validity}. To score the SIPAS, the overall mean of the ratings on a 6-point Likert scale with a higher score indicating a stronger agreement is taken. We replaced "system" with "AI system" for all items.
%\todo{Appendix: \textit{It was transparent to me which information was collected by the AI system (1), The information that the AI system could acquire was observable for me (2), It was understandable to me how the collected information led to the result (3), The AI system's information processing was comprehensible to me (4), With the information accessible for me, the result was foreseeable for me (5), The AI system's information processing was predictable for me (6).}}
% \paragraph{Meta AI Literacy Scale}
% In order to assess the participants' knowledge of AI, we distributed the Meta AI Literacy Scale (MAILS). This scale measures AI literacy in various areas such as \textit{Use and apply AI}, \textit{Know and Understand AI}, \textit{Detect AI}, and \textit{AI Ethics}. It also includes separate constructs to evaluate one's ability to \textit{Create AI}, \textit{AI Self-efficacy in problem solving and learning} and \textit{AI Self-competency}. For our study, we only used the 18 items related to AI literacy facets. Participants rated their knowledge on an 11-point Likert scale, ranging from 0 (not at all) to 10 (very well) \cite{Carolus_2023_MAILS}. The scores for all items were summed up to provide an overall AI literacy score on a scale of 0 to 180.

%\todo{Appendix: I can operate AI applications in everyday life. I can use AI applications to make my everyday life easier. I can use artificial intelligence meaningfully to achieve my everyday goals. In everyday life, I can interact with AI in a way that makes my tasks easier. In everyday life, I can work together gainfully with an artificial intelligence. I can communicate gainfully with artificial intelligence in everyday life. I know the most important concepts of the topic "artificial intelligence". I know definitions of artificial intelligence. I can assess what the limitations and opportunities of using an AI are.}

% \paragraph{Checklist for trust between people and automation}
% To measure the participant’s trust in the AI system, we utilized the Checklist for Trust between People and Automation (TPA) \cite{jian_2000_Trust_Automated_Systems}, which uses distrust and trust as polar opposites of one dimension \cite{Kohn_2021_TIA_validation}. It has previously been used to as an attitudinal measure of trust in AI systems \cite{Scharowski_2023_Effecst_AI_explanations_trust_reliance}. The TPA uses a 7-point Likert scale ranging from 1 (not at all) to 7 (extremely) and contains 12 items. To score the TPA, the first 5 items sampling distrust are reverse coded and all of the items are summed up for an overall trust score. The psychometric properties of TPA have been evaluated \cite{Spain_TPA_evaluated} and it has also been validated in German \cite{pohler_2016_Trust_Automated_Systems_german_validation}.

%\todo{Appendix? items: The system is deceptive, The system behaves in an underhanded manner, I am suspicious of the system's intent, action or outputs, I am wary of the system, The system's actions will have a harmful or injurious outcome, I am confident in the system, The system provides security, The system has integrity, The system is dependable, The system is reliable, I can trust the system, I am familiar with the system}

% \paragraph{Manipulation Check}
% The Manipulation was assessed with the question \textit{Did you believe that an AI system was implemented to adapt task pace?} The possible answers were \textit{Yes, No} or \textit{Partially}. If the participant checked partially, they were asked to specify and elaborate on why they only partly believed that an AI system was implemented. Participants were also allowed to comment on why they did or did not believe in the AI system in the same specification field. 


%\subsection{Data analysis}
% \paragraph{EDA pre-processing}

% Skin conductance responses were processed after the experiment using the open-source Neurokit Python library~\cite{makowski2021neurokit2}. We applied a low-pass Butterworth filter (cutoff = 3\,Hz, order = 4) to the EDA data alongside a convolutional smoothing filter. The processed EDA signal was then decomposed into its phasic and tonic components using median subtraction following the AcqKnowledge procedure~\cite{braithwaite2013guide}. The tonic component of the EDA signal is a low-frequency oscillation that serves as an indicator of general arousal with a slow and inertial response. The phasic component on the other side, consists of higher frequency oscillations in the EDA signal that typically relate to discrete events. 

% As an indicator for the tonic skin conductance response we...%
% As there is no fixed onset of the stimulus, we extracted the maximum phasic response amplitude for each agent from the phasic EDA signal within a response window of %adapt this

% .  Following the standardized  Neurokit pipeline~\cite{makowski2021neurokit2}, we extracted all peaks in the smoothed phasic component with a minimum amplitude of .001\,$\mu$V ~\cite{cartaud2018physiological}. 


% We use a Bayesian approach to data analysis for this paper. We used Bayesian linear mixed models (BLMM). The Bayesian approach has been taken up lately  \cite{kay2016researcher,kay2016special, URBANIAK2022107371,ACKERMANS2019248,GUERONSELA2023107572} as it presents several advantages to classical statistics. \citet{kay2016researcher} explain the advantages of Bayesian statistics in technological contexts that are also relevant to our study. These are, in particular: 1. The ability to use prior knowledge and learn from data. 2. To inform on the size of the placebo effect with a given level of precision, 3. It allows for the estimation of effects in small n-studies, 4. The approach enables readers to evaluate the effect size, which can also be close to zero, rather than the mere effect existence. For a tutorial on Bayesian statistics, a description of the common workflow using brms, and reporting guidelines, see \cite{schad2021toward,van2021bayesian,dix2022bayesian, burkner2017brms}. Most importantly, an effect's existence and non-existence are likewise important. The Bayesian approach to statistical inference allows us to measure the placebo/nocebo effect and their absence on the measures.
% Here, we use Bayesian parameter estimation which allows us to estimate parameter values of effect sizes and quantify the uncertainty regarding these estimates based on the information in our data and the priors applied. We used brms~\cite{burkner2017brms}, a wrapper for the STAN-sampler \cite{carpenter2017stan}. For statistical inference, we used R \cite{R-base} along with packages for preprocessing \cite{tidyverse2019,R-Matrix,R-here,R-haven,R-readr}, modeling \cite{R-brms,brms2017,lme42015,lmerTest2017,R-psych,Rcpp2011} and post-processing \cite{R-tidybayes,R-apa,R-bayestestR,ggplot22016,knitr2015,R-extrafont,R-patchwork,see2021,R-sjstats} the data. We computed 4 Hamilton-Monte-Carlo chains with 40000 iterations each and 20\% warm-up samples. Trace plots of the Markov-chain Monte-Carlo permutations were inspected for divergent transitions. %All Rubin-Gelman statistics~\cite{gelman1992inference} were well below 1.1, for effective sampling size.

% We compare possible models with approximate leave-one-out cross-validation (LOOCV) \cite{vehtari2017practical}. This procedure allows us to compare information criteria across models. Relatively smaller LOOCV values indicate a better fit of the model to the data. The best model is then selected and parameters are further analyzed. For these, $p_b$ was computed by calculating the relative proportion of posterior samples being zero or opposite to the median. This metric has similar properties to the classical \textit{p}-value ~\cite{hoijtink2018testing,meng1994posterior,shi2020reconnecting} but quantifies the proportion of probability that the effect is zero or opposite given the data observed. Note that this is the reverse of the classical approach to inferential statistics, where one measures the probability of the data given the null-hypothesis with respect to the test statistic. Effects were considered meaningful when there was a particularly low probability ($p_b$ <= 2.5\%) of the effect being zero or the opposite.
% In addition to the median of the parameter, we calculated the High-Density Interval (HDI) at 95\% of the posterior distribution for all parameters, which indicates the possible range of effects given the data, alongside the median of the respective parameter. Simple mean comparisons were made on standardized outcome variables. Therefore, all $\tilde{b}$ represent an effect size in terms of deviations of the standard deviations from the mean (corresponding to Cohen's D for simple effects of categorical predictors with two levels). For models on factorial designs, our analysis of the physiological data, we calculated $\delta_t$, which can be interpreted quite similar to Cohen’s d and is based on standardizing the population-level effects on the varying-effects and residual variance  \cite{judd2017experiments,hedges2007effect}. For the behavioral responses we will fit a hierarchical 3-parameter drift-diffusion model (bias = 50\%) that predicts the non-decision time, drift rate and decision-boundary for each condition. 

%results without contrasted factors
%Participants were asked to indicate if they thought they would perform better with the sham AI system on a scale ranging from 1 (strongly disagree) to 7 (strongly agree). Participants in the placebo group indicated a stronger agreement for performing better with the sham AI system active ($M$ = 4.78, $SD$ = 0.99) than the nocebo group ($M$ = 4.32, $SD$ = 1.16). This difference could be distinguished from zero $\tilde{b}_\text{group}$=  0.78  [0.07, 1.46] , $p_b$ = 1.35\%,  $\tilde{\delta}_\text{b}$=  0.55 [0.07, 1.05]. Participants showed a stronger agreement with performing better with the sham AI system before interacting with the sham AI system ($M$ = 4.74, $SD$ = 1.09) than after the interaction ($M$ = 4.35, $SD$ = 1.66). This difference could be distinguished from zero $\tilde{b}_\text{condition}$=  0.69  [0.08, 1.32] , $p_b$ = 1,4\%,  $\tilde{\delta}_\text{b}$=  0.49 [0.05,  0.93].



%results without contrasted factors
%Another scale assessed the participants' expected correct identifications with and without the sham AI system active. For this, the participants were asked to indicate how many points they thought they would score with and without the sham AI system on a scale ranging from 0 to 200 points. Participants in the placebo group indicated that in the AI condition ($M$ = 145, $SD$ = 36.5), they will score more points than the no-AI condition ($M$ = 132, $SD$ = 34.1). This difference could be distinguished from zero $\tilde{b}_\text{condition}$=  15.06  [0.61,  29.76] , $p_b$ = 2.07\%,  $\tilde{\delta}_\text{b}$=  0.37 [0.01,  0.73]. Participants in the nocebo group showed no significant difference between the AI and no-AI conditions.

%results without contrasted factors
%A regression model was computed to assess the expected task speed of the participants with and without the sham AI system active with \textsc{condition} (assessment before and after interaction) and \textsc{group} as predictors and an intercept of 50. We found no significant differences for \textsc{condition} $\tilde{b}_\text{std}$ = 5.64 [-2.75, 14.32], $p_b$ = 9.65\%, \textsc{group} $\tilde{b}_\text{std}$ = 0.28 [-8.41,  9.28], $p_b$ = 47.53\% or interaction effects $\tilde{b}_\text{std}$ = 4.69 [-7.49, 17.01], $p_b$ = 22,47\%. We can conclude that neither the \textsc{condition: pre/post} nor the \textsc{group} has a significant effect on the expected task speed.

% All estimated population-level parameters can be found in ..... 

% We find that the model makes similar predictions as 


% \begin{table}[tbh]
% \caption{Model outputs for the parameters on the log scale. Confidence intervals at the 95\% level are provided for each parameter, along with their medians.}
% \begin{tabular}{llcll}
% \toprule
% Parameter & Median & $HDI_\text{95\%}$ & $\hat{R}$ & ESS \\ 
% \midrule
% \textit{Drift-rate AI} & -2.66 & [-3.22, -2.09]  & 1.003 & 328.00 \\
% \textit{Drift-rate Control} & -2.63 & [-3.22, -1.99] & 1.006 & 431.00 \\
% \textit{Boundary-seperation AI} & 1.36 & [1.25, 1.47]  & 0.999 & 1186.00 \\
% \textit{Boundary-seperation Control} & 1.43 & [1.31, 1.58]  & 0.999 & 1206.00 \\
% \textit{Non-decision time AI} & 0.34 & [0.32, 0.36]  & 1.001 & 843.00 \\
% \textit{Non-decision time Control} & 0.34 & [0.31, 0.36]  & 0.999 & 936.00 \\
% \textit{Bias AI} & 0.31 & [0.17, 0.45]  & 1.001 & 903.00 \\
% \textit{Bias Control} & 0.38 & [0.20, 0.55] & 1.003 & 874.00 \\
% \bottomrule
% \end{tabular}
% \label{tab:model-outputs}
% \end{table}


% \begin{figure}[tbh]
%     \centering
%     \includegraphics[width=0.5\textwidth]{diff_nocebo_plot.pdf}
%     \caption{ Posterior density plot for the difference in parameter values for Drift-rate and boundary separation in our Nocebo model.}
%     \label{fig:paramdiffnocebo}
% \end{figure}


% \begin{figure}[tbh]
%     \centering
%     \includegraphics[width=0.9\textwidth]{RTplot_nocebo.pdf}
%     \caption{A: Mean reaction time with error bars denoting +/- one standard error of the mean as a function of condition (Nocebo AI vs. Control) and correctness of trial (correct in green, incorrect in red). B:Posterior density plot for the difference in parameter values for Drift-rate and boundary separation in our Nocebo model. }
%     \label{fig:paramdiffnocebo}
% \end{figure}

% \begin{figure}[tbh]
%     \centering
%     \includegraphics[width=0.9\textwidth]{suspcicion_deception.pdf}
%     \caption{A: Posterior difference for proportions of failed deception across groups (nocebo-placebo). B: Posterior difference for proportions of suspicion across groups (nocebo-placebo)}
%     \label{fig:tlx_sum}
% \end

%We compared the average NASA TLX Raw sum score across \textsc{description}. There was no significant difference between conditions, $\tilde{b}_\text{std}$= -0.03  [-0.09, 0.04], $p_b$ = 21.96\%. Looking closely at the posterior distribution of the mean difference (Figure \ref{fig:tlx_sum}) and taking into account the $HDI_\text{95\%}$, it is highly unlikely that the \textsc{augmentation} condition produced any kind of increased subjective workload in the TLX. The $HDI_\text{95\%}$ indicates that any difference would be smaller than around 1/10 of a point on the sum-score. We can follow that the effect of the \textsc{description} on the TLX is negligible and not distinguishable from a null-effect. We also found no effect on any of the TLX-subscales, all $p_b$ > 5.23\%


% \subsection{Task Load}
% \begin{figure}[tbh]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Content/tlx_plot.pdf}
%     \caption{\ColorPrint A: Average TLX sum score with connected individual mean values. Error bars denote ±1 standard error of the mean. B: Prior and posterior density plots. Prior samples in beige, and posterior samples in green. The relative density increase from prior to posterior shows how the data has informed the model.  Posterior samples are centered at zero, indicating that the effect is likely to be small, or zero.}
%     \label{fig:tlx_sum}
% \end{figure}

\subsection{Qualitative themes}
- cluster of partially believed answers

%Here, we present the findings of our qualitative inquiry. Based on our analysis, we conceptualized six dimensions: \textsc{Peril}, \textsc{Privacy}, \textsc{Access}, \textsc{Motivation}, \textsc{Ownership}, and \textsc{Achievement}, plus an overarching topic consistently found in the interviews, which is the \textsc{Personal} preference to have an augmentation. Our findings are described below and illustrated with excerpts from the interviews. Each excerpt is marked with the respective participant ID. %

%\subsection{Peril \& Privacy}
%The first theme focused on the potential danger emanating from human augmentations, encompassing aspects such as human augmentations as weapons or invisible threats, privacy issues, and defense strategies. Interestingly, participants considered the potential risks of human augmentation from different perspectives. Risks caused by AHs as well as risks caused by the actual augmentation were discussed. The fact that it was unclear who or what was the source of risk in human augmentations (e.g., the human or the technology) and who could possibly be harmed by the augmentation (e.g., the augmented human or a non-augmented human) illustrates the complexity of the issue. The need to assess the risks posed to the AHs by the augmentation was emphasized by many participants. The following statement highlights this consideration:
%\begin{quote}
%   For public use, the legal side of it should be checked (...) that person that is going to be using it, is this [i.e., the augmentation] going to pose any kind of threat to their body or physiology. I would like to check all this first, then I'll go for that. (U4) 
%\end{quote}

%All participants discussed the potential threat to individuals or society caused by different augmentations. For example, they often either explicitly or implicitly compared them to weapons. This is highlighted by a statement of one participant discussing the potential danger of bionic vision compared with a motor augmentation:
%\begin{quote}
  %  When it comes to bionic vision, yes, it could interfere, but in this case (motor augmentation), it shouldn’t unless this person does, I don’t know, some sort of martial art. Their legs would allow this person to give a faster kick or a better punch. They would be stronger and hurt the person they’re fighting against.
%It could also be dangerous because having such strong legs could lead you to kill someone by simply kicking them. (C1)
%\end{quote}

%It appears that participants carry their rich everyday experiences and their narratives of AI to the evaluation situation, biasing their subjective evaluations and their behavior. These cannot be overruled by simple verbal descriptions, invalidating some placebo mechanisms presented in the HCI literature \citet{kosch2022placebo,villa2023placebo}.

==> old_text.tex <==

% Individuals who use AI systems to support decision-making often outperform those who do not. Yet, a recent study~\cite{villa2023placebo} discovered that individuals make riskier decisions when they hold high expectations of performance of an AI system, even if the AI system is non-functional. This underscores two key points: first, the influence of expectations on the interaction with AI systems and the decision-making process; and second, the need to align these expectations with the actual system capabilities. 

% Analog to the medical field, administering a sham treatment (e.g., a placebo) can elicit patient anticipations of improvement, subsequently enhancing a patient's condition even in the absence of any active substance or specific medical procedure. Such a placebo can alleviate pain~\cite{lasagna1954study} or support the treatment of ailments \cite{beecher1955powerful}. Similarly, negative expectations on treatment outcomes can impair medical treatment and potentially worsen a patient's condition \cite{enck2019does,jensen2012nonconscious} -- a phenomenon known as the nocebo effect. Consequently, aside from the treatment itself, people's expectations~\cite{stewart2004placebo,lasagna1954study, montgomery1996mechanisms} significantly influence study outcomes and thus can undermine scientific evaluation.


% Although useful for treatment, the placebo effect obscures treatments' assessment, making dedicated control conditions necessary \cite{Price2008ACR} as large sample sizes, randomization and blinding can often not mitigate these effects.  

% Contrary to our goal of testing the consequences of negative expectations, we were unable to induce negative expectations through verbal descriptions. Interestingly, we found that regardless of positive or negative AI descriptions, participant's reaction times were faster when they believed that an AI support system was present. 
% Further, we used a widely used cognitive modeling technique called drift-diffusion model (DDM) to analyze the decision-making process. We found that participants gathered information quicker in the AI condition (as described by the v factor of the DDM) compared to the control condition and that they did not change their response strategy in the process (e.g. prioritizing speed over accuracy).
% %Cognitive modeling, with the drift-diffusion model, revealed that in the AI condition, participants gathered information faster as compared to the control condition and that they did not change their response strategy, e.g., prioritize speed over accuracy in the AI condition. 
% This is mirrored in the subjective feedback of participants regarding the usability of the system, user experience and ease of the task. However, we did not find any effect of our manipulations on subjective workload or physiological indicators of workload (EDA). In a second study, we aimed to replicate the impact of negative verbal descriptions of AI. % and assess  its robustness. %By analyzing quantitative and qualitative user responses of users anticipating using a similar AI system, 
% We found that even if users explicitly acknowledged that the AI decreased task performance for other users, they did not expect their own performance to decline accordingly; validating the robustness of AI to negative verbal descriptions.

%\todo{work in progress... add studies on large divergence on expectations (future scenarios), individual differences, important aspects for trust in AI, what do people want in AI systems, how could AI futures look; more real life application studies, get to the point}

% \textbf{However, the influence of such narratives on individual technology use and interaction remains an open question.}
% The perceptions individuals have about technology can greatly influence their usage %\cite{KING2006740}
% . Prior research has delved into several key concepts such as people's expectations regarding transparency \cite{meurisch_exploring_2020,park_human-ai_2021,purcell_fears_2023}, the relationship between humans and AI \cite{zhang_ideal_2021}, and autonomy \cite{meurisch_exploring_2020}. These concepts form the foundation for designing AI interfaces. Yet, there is a noticeable knowledge gap regarding expectations of outcomes for Human-AI interactions, for example, how people anticipate they will perform a task with AI-support\cite{kosch2022placebo}.
% There are some indications on these expectations in large-scale surveys. In 2019, Cave and Dihal conducted a study examining people's hopes and fears about AI within the British population, informed by depictions in Western media and fiction \cite{cave2019hopes}. They found that the anxiety about the potential disruptive impact of AI outweighed the excitement within the general population. Particularly, individuals expressed fear of obsolescence and alienation; in other words, they were worried about AI negatively influencing their work and personal relationships \cite{cave2019scary}.
% These findings align with those of Sartori et al. (2023), who reported a higher incidence of AI-related worries than perceived benefits, a phenomenon they termed as 'AI anxiety' \cite{sartori_minding_2023}. Various factors have been suggested to explain this imbalance, including the portrayal of AI technologies in science fiction \cite{hermann2020beware}. It's important to note, however, that the narratives surrounding AI can vary depending on stakeholders and evolve over time \cite{bory2019deep}.Thus, expectations surrounding AI outcomes are not perfectly balanced but at times lean towards the negative, perhaps influenced by prevalent societal narratives about AI \cite{hermann2020beware,bory2019deep,cave2019scary}.

% AI narratives are vastly influential. 
% For instance, national science and business policies in countries such as China, Germany, the USA, and France now emphasize the disruptive potential of AI \cite{bareis2022talking}. Indeed experts deem that these AI narratives are influential on many levels  \cite{bory2019deep}
% %people warning about the impact of AI narratives https://link.springer.com/article/10.1007/s00146-022-01548-2#ref-CR15    
% \textbf{Yet, the impact of these narrative-driven expectations on individual use and interaction with technology remains unclear and thus needs to be investigated.}
% \citet{lasagna1954study} laid the groundwork for research on placebo effects, which involve symptom alleviation due to patient expectations \cite{Price2008ACR}. Such effects have been confirmed in both clinical and psychological settings \cite{Hrbjartsson2001IsTP, Diederich2008ThePT}. While placebo treatments have broad applications, they most consistently improve subjective outcomes \cite{Beckham1989ImprovementAE, Rickels1970Pills}.

% Decision-making is a fundamental part of human behavior, which is heavily impacted by our expectations and perceptions. It is usually described as the act of selecting one option from a variety of alternatives \citep{SHAFIR199311}. The Drift Diffusion Model (DDM) is a cognitive model that is commonly used to explain decision-making \cite{ratcliff_perceptual_2010,ratcliff_rouder_2000_dm_2C_Letteridentification}. This model portrays decision-making as a process in which evidence is accumulated until a decision boundary is reached. The drift rate quantifies the speed of information gathering, while the decision boundary symbolizes the amount of information needed to make a certain decision. To improve this model, a non-decision time and a decision bias are often added, which represent a prior in location and time for initiating the evidence accumulation process. This model has been successful in predicting decision-making under uncertainty and in different cognitive tasks \cite{ratcliff_perceptual_2010,ratcliff_rouder_2000_dm_2C_Letteridentification} and can explain how people make a tradeoff between accuracy and speed when making decisions. The DDM has a wide range of applications, from HCI topics such as pedestrian crossing \cite{zgonnikov2022should}, moving target selection \citet{lee2018moving}, to interactions with robots \cite{huang2020human} or teleoperations \cite{corredor2016decision} and is used to model the decision process for HCI applications %\citet{https://content.iospress.com/articles/journal-of-intelligent-and-fuzzy-systems/ifs179548}.

% AI has added a new layer to the decision-making process of computing systems initially in the form of AI synthesizing or augmenting decision making by improving data quality, \citet{beede2020human, abidi2006improving, ingrams2022ai} .


% More recently, however, AI has been integrated into user interface design ~\cite{HORNBAEK200679,browne2016adaptive}, aiding users in decision-making by delivering relevant information at opportune moments or the right location and lessening decreasing cognitive load through interface adjustments based on physiological signals \cite{koschrsvp,kosch2019your}. This paradigm shift focuses not on altering information quality but on improving the interface for accessing information. \citet{kosch2022placebo} has found that mere descriptions of a sham adaptive AI can affect performance (placebo effect). They found that participants that believed an adaptive AI will support them would  produced more accurate performance. \citet{villa2023placebo} could show that this has an impact on risky decision-making. A sham adaptive AI-based cognitive enhancement made participants take more risks in a standardized card game. Thus, technologies can serve as a placebo that improves performance in tasks and decision making contexts. Note that so far the cognitive basis of these effects are unclear.

% In HCI, AI initially augmented decision-making by enhancing data quality \cite{beede2020human, abidi2006improving, ingrams2022ai}. Recently, its role has shifted towards being integrated into user interface design to assist users in making decisions \cite{HORNBAEK200679,browne2016adaptive}. This new focus is on optimizing the interface for better information access, aligning closely with the DDM's emphasis on the quality and speed of decision-making.


%Although previous work successfully demonstrated placebo effects in HCI, nocebo effects have received little attention in HCI research. We argue that much like unwarranted positive expectations with regard to AI can produce placebo effects \cite{kosch2022placebo}, it appears plausible that likewise negative expectations stemming from preconceptions of AI \cite{cave2019scary} could worsen performance. A nocebo effect potentially biases conclusions in novel and high-expectancy areas such as interaction with AI. We address this research gap by presenting one experiment investigating the impact of user expectations and nocebo effects on user experience measures and decision-making.

%Previous research has shown that social learning \cite{kirsch1999specifying}, classical conditioning \cite{flaten1999caffeine}, or verbal information (e.g., expert instructions \cite{stewart2004placebo}) can all be used to generate placebo responses. We concentrated on the latter and 
 %we manipulated expectations by changing system descriptions \citep{kosch2022placebo}.
% In line with \citet {kosch2022placebo}, we conducted a within-subjects to determine the effect of manipulating positive and negative AI expectations on decision-making and thus their propensity to have placebo and nocebo response. We operationalized decision-making through the letter discrimination task. %In the sham-AI condition, participants were told an AI system would be in place that would increase (placebo) or impair (nocebo) their performance. In the control condition, participants were told the AI system was turned off.


% \noindent \textbf{RQ1:} Do subjective ratings on performance and mental workload differ between negative and positive verbal descriptions (nocebo/placebo)?

% \begin{itemize}
%     \item \textbf{H1:} For sham AI with a negative description (nocebo) participants will report a lower subjective performance before and after interaction and a higher mental workload after interaction when compared to a control condition.
%     \item \textbf{H2:} For sham AI with a positive description (placebo) participants will report a higher subjective performance before and after interaction and a lower mental workload after interaction when compared to a control condition.
% \end{itemize}

% \noindent \textbf{RQ2:} Do verbal descriptions affect decision-making (e.g., in a letter discrimination task)?

% \begin{itemize}
%     \item \textbf{H3:} For a sham AI condition with a negative description (nocebo), the speed-accuracy trade-off parametrized by boundary separation is more conservative in comparison to a control condition.
%     \item \textbf{H4:} For a sham AI condition with a positive description (placebo), the speed-accuracy trade-off parametrized by boundary separation is more liberal in comparison to the control condition.
% \end{itemize}


% \noindent \textbf{RQ3:} Do verbal descriptions in a sham condition affect physiological indicators of cognition when compared to a control?

% \begin{itemize}
%     \item \textbf{H5:} When comparing a sham AI condition with a negative description (nocebo) to a control condition, the sham condition will show higher levels of physiological arousal measured by mean tonic skin conductance level (SCL).
%     \item \textbf{H6:} A sham AI condition with a positive description condition will show lower levels of physiological arousal measured by mean SCL than the control condition.
% \end{itemize}

% Performance expectations concerning the AI system were gauged both before and after the interaction. We utilized a Likert scale for this assessment, along with explicit metrics like anticipated speed and the number of correct responses forecasted. To quantify mental workload, we'll employ EDA measurements in tandem with the NASA-TLX post-interactions.

% Key parameters for decision-making are rooted in the reaction times and accuracy derived from the letter discrimination task  \cite{ratcliff_perceptual_2010}, where participants see a letter on a screen and have to press a pre-specified button as fast as possible. This task, a standard in psychological decision-making research, has been adapted to study domains as demanding as air traffic control %\cite{https://link.springer.com/chapter/10.1007/978-3-642-39215-3_62}          .
% Our selection of the letter discrimination task is informed by its potential to simulate the rapid information processing and decision-making that typify brisk human-computer interactions.
%It was based on the experiments conducted by \cite{thapar_2003_Letter_discrimination_task} and was implemented using lab.js \cite{henninger_2021_labjs}.

%This mask was implemented to increase the task's difficulty by reducing the amount of information available from the stimulus % literature in macaques\cite{rolls_1999_backward_masking}, looking for human studies. re-write: this is done in psychology research to mask the effect of the target stimulus, so participant can't remember and actively has to make a choice --> cite studies.

% \paragraph{System Usability Scale}
% To assess the usability of the AI system, we utilized the System Usability Scale (SUS) \cite{Brooke_SUS_1995}. This questionnaire is a reliable and validated tool that measures the subjective usability of technological systems \cite{Brooke_SUS_retrospective, peres_2013_SUS_validation}.  The usability score is computed by calculating the weighted sum score. In line with \citet{Finstad_SUS_non-native-speaker}, we adapted the SUS by specifying that the system being evaluated is an "AI system" and added the synonym \textit{awkward} in addition to \textit{cumbersome} \cite{Finstad_SUS_non-native-speaker}.
% %\todo{Appendix: \textit{I think that I would like to use this AI system frequently (1), I found the AI system unnecessarily complex (2), I thought the AI system was easy to use (3), I think that I would need the support of a technical person to be able to use this AI system (4), I found the various functions in this AI system were well integrated (5), I thought there was too much inconsistency in this AI system (6), I would imagine that most people would learn to use this AI system very quickly (7), I found the AI system very cumbersome (awkward) to use (8), I felt very confident using the AI system (9), I needed to learn a lot of things before I could get going with this AI system (10).}}


% \paragraph{Short Version of the User Experience Questionnaire}
% The is a shorter version of the user experience questionnaire, containing only 8 items (Likert scale from -3 to +3). It assesses two dimensions out of the original three dimensions (attractiveness, pragmatic quality and hedonic quality) related to usability: pragmatic quality, e.g., efficiency, perspicuity, and dependability) and hedonic quality, e.g., stimulation and novelty. Scales can be calculated by averaging across items. %The items are taken equally from both the pragmatic and hedonic quality scales, with pragmatic items presented first, followed by hedonic items. 
% %Each item was rated on a 7-point-Likert scale from -3 to +3, indicating stronger agreement with negative terms on the left or positive terms on the right. %TThe overall UX value is calculated by taking the mean of the eight items. %The UEQ-S is available in multiple languages and psychometrically validated \cite{Schrepp_2017_UEQS}.
% %\todo{Appendix: \textit{obstructive vs. supportive, complicated vs. easy, inefficient vs. efficient, confusing vs. clear, boring vs. exciting, not interesting vs. interesting, conventional vs. inventive, usual vs. leading edge}}
 %We identified nsSCRs peaks using a .05 mS threshold value, following the recommendations by the Society for Psychophysiological Research ~\cite{society2012publication}.

%We manipulated participant's expectations in a letter discrimination task (e.g., see \cite{ratcliff_perceptual_2010}) by altering the \textsc{system description}  %(i.e., \textsc{nocebo} condition vs. \textsc{placebo} condition) 
%and \textsc{system status}.% In detail:%(i.e., \textsc{sham AI condition} condition vs. \textsc{no-AI} condition). 
%To the participants, the \textsc{system status} was shown on the monitor as \textit{AI active} (\textsc{sham AI}) and \textit{AI inactive} (\textsc{no-AI}). %The participants were blinded with regard to other groups. 

%The \textsc{system description} was manipulated to either have a negative (\textsc{nocebo}) or positive (\textsc{placebo}) influence on the participant's perception of the AI system. 


% To characterize the samples perception of our sham AI system and automated systems in general we have employed three additional scales. First, the Subjective Information Processing Awareness Scale (SIPAS) is a questionnaire that assesses how users perceive, understand, and predict information processing when interacting with intelligent systems in a short-form \cite{Schrills_Franke_2021_SIPAS, Schrills_2021_SIPAS_validation, Schrills_Franke_2023_SIPAS_validity}. We replaced "system" with "AI system" for all items and scored it by taking the overall mean for each participant. Second,  to assess the participants' knowledge of AI, we distributed the  AI literacy-related items of the Meta AI Literacy Scale (MAILS; 11-point Likert scale, ranging from 0 - not at all to 10 - very well; sum-scored) \cite{Carolus_2023_MAILS}. Third, to measure the participant’s trust in the AI system, we utilized the Checklist for Trust between People and Automation (TPA) \cite{jian_2000_Trust_Automated_Systems}, which uses distrust and trust as polar opposites of one dimension \cite{Kohn_2021_TIA_validation} (7-point Likert scale ranging from 1 - not at all to 7 - extremely; sum-scored). 

% \begin{table}[h]
% \centering
% \caption{Participant Demographics and Scores by Group}
% \begin{tabular}{lcccc}
% \toprule
% Group & Females & Males & Average Age ($M \pm SD$) & Technical Competence ($M \pm SD$) \\
% \midrule
% Positive System Description & 20 & 12 & $27.58 \pm 6.24$ & $5.03 \pm 1.15$ \\
% Negative System Description & 20 & 13 & $27.58 \pm 6.82$ & $4.61 \pm 1.32$ \\
% \bottomrule
% \end{tabular}
% \end{table}
% \FloatBarrier

%The group with the positive system description consisted of 20 female and 12 male participants, with an average age of 27.58 years ($M$ = 27.58, $SD$ = 6.24) and a technical competence score of 5.03 out of 7 ($M$ = 5.03, $SD$ = 1.15) on a Likert scale. The group with the negative system description consisted of 20 female and 13 male participants, with an average age of 27.58 years ($M$ = 27.58, $SD$ = 6.82) and a technical competence score of 5.03 out of 7 ($M$ = 4.61, $SD$ = 1.32) on a Likert scale.


% \subsubsection*{System status}
% Participants were asked to assess an adaptive AI system used in a letter discrimination task. They were also informed that they would need to perform the same task without AI assistance later. 
% In the \textsc{sham AI} condition, participants were informed %of people performing more efficiently when the task difficulty level fits their stress level. Therefore, 
% that a research team had developed an AI system that adjusts task difficulty in reaction-critical contexts by analyzing the user behavior and electrodermal activity measured using electrodes in two fingers of their non-dominant hand. Then, the AI system would dynamically adjust the task's difficulty by altering the task's pace according to the measured stress level and task performance.  Participants were informed that it might take some time to notice these pace adjustments. 
% \todog{Make the no-AI vs Control naming convention consistent}
% In contrast. in the \textsc{no-AI} condition, participants were informed that the AI system was not active and that the task pace was random. Therefore, their performance in the letter discrimination task would not be influenced by the AI system. The purpose of this condition was to act as a control condition in our experiment. It is important to highlight that the description of the adaptive AI system presented in this study is purely fictional. There was no adaptive AI system in place.

%The experimenter then went behind a room divider and recorded the group, room temperature, and humidity and filled in the participant ID.
%Participant group allocation and condition order was counterbalanced to avoid order effects. Participant screening was done as described in \autoref{sec:p1}.

%\subsubsection*{Pre-experimental procedure}
%Upon arrival, the participants were provided with details about the study's goals, procedure, and data protection. Subsequently, they requested to authorize the use of their data in compliance with the Declaration of Helsinki.
%\subsubsection*{Starting the experiment \& Demographic information}

%\subsubsection*{Explaining the AI system}

%Then, The experimenter instructed the participant to read all instructions and questions thoroughly. 
%Participants were allowed to ask any questions, take breaks between the tasks and withdraw their consent at any point. 
%However, the AI system implemented in our study was a sham system and, therefore, not operational. 
%We followed the methods used in previous studies investigating a placebo effect in HCI \cite{villa2023placebo, kosch2022placebo} to induce a nocebo and placebo effect.% Finally, Participants read a description of an adaptive AI system that adjusts task difficulty in reaction-critical situations. This system was presented as an EDA-based AI that adapts pace according to an individual's stress response.
%After the description, we made sure participants took up all relevant information using three rephrased questions previously implemented in \citet{villa2023placebo}.%: \textit{Which two conditions are you testing in this study?}, \textit{What is the intent of the use of the AI system in this study?}, and, \textit{What is the collected data used for?}. Each item had three possible response options, but only one was correct.
%\todo{All participants included in the study answered these questions correctly.??}\todo{(See supplementary material: \*OSF??), add questions in appendix?}

%\subsubsection*{Task instructions}
%After study comprehension was assessed, instructions for the letter discrimination task were presented on the screen, along with an example figure of the task. Participants were informed about the conditions again. Then, they were instructed to respond as quickly as possible to every letter displayed, even if they were unsure of the correct identification. 

% \subsubsection{Sham calibration - practice block}
% Participants were informed about the conditions again. Then, they were instructed to respond as quickly as possible to every letter displayed, even if they were unsure of the correct identification. 
% Then, participants performed a sham AI system calibration block, which simultaneously served as a practice block.
% This calibration involved 50 trials. During these trials, they received visual feedback on their performance through colored stimuli (correct --> green, incorrect -->red). 
% Following this, we polled participants' expectations of their performance with and without the AI system were assessed.

%\subsubsection*{Performing the task}

%The conditions were counterbalanced to avoid effects caused by experimental order. Depending on whether the AI system status was apparently active (sham-AI) or inactive (no-AI), the participant received a notification on the system status on their screen. If the AI was active, it stated that the AI would monitor their progress and adjust the pace of the task. They were also given a short written and verbal system description (nocebo or placebo), followed by a loading screen for 20 seconds, indicating that the AI calibration was being retrieved. If the AI was inactive, they were informed that their performance would be assessed without the AI system, and the task pace would be random. In both cases, they were reminded to keep their hand with the electrodes facing upward. 
% We additionally obtained time-series data using the Lab Streaming Layer (LSL) for networking, time synchronization and recording EDA from Bitalino. The participants filled in questionnaires and performed the tasks using a digital experiment environment developed with JavaScript using the lab.js library version 20.2.4 \cite{henninger_2021_labjs}. 
% Markers for EDA analysis were sent at the beginning and end of each trial set (100 trials) via HTTP to a Python server that forwarded them to the LSL network. All of the system components were run locally.


%Recent literature emphasizes the Bayesian approach's advantages, such as incorporating prior knowledge, precisely determining the placebo effect's magnitude, facilitating effect estimation in small sample sizes, and providing an effect size evaluation \cite{kay2016researcher,URBANIAK2022107371,ACKERMANS2019248,GUERONSELA2023107572}. Notably, it allows both the identification and absence of effects to be equally informative \cite{kay2016researcher}.

%For simple two-level mean comparisons, we standardized outcomes, all $\tilde{b}$ denoting effect sizes analogous to Cohen's D. 
%We used $\delta_t$ for effect size, akin to Cohen’s d \cite{judd2017experiments,hedges2007effect} for model parameters in linear regression models. %Behavioral responses were analyzed using a hierarchical 3-parameter drift-diffusion model implemented in brms \cite{burkner2017brms}.

%Model comparison was conducted via leave-one-out cross-validation (LOOCV) \cite{vehtari2017practical}, where smaller LOOCV values denote superior model fit. Selected 

%Another scale assessed the participants' expected correct identifications with and without the sham AI system active. For this, the participants were asked to indicate how many points they thought they would score with and without the sham AI system on a scale ranging from 0 to 200 points. 

%We can follow that the effect of \textsc{system description} and all interaction effects between \textsc{system description}, \textsc{system status} and \textsc{time} on the expected task speed is negligible and not distinguishable from zero.

%Then, we modeled reaction time in seconds as a function of \textsc{system status} with varying intercept and varying slopes for the condition in each participant (LOO = -26363.3) and compared it to a model that also had \textsc{System description} and their interaction as predictors (LOO =-26364.1). We selected the most complex model with both \textsc{System status} and \textsc{System description} as it allows us to quantify the absence effect of a placebo/nocebo distinction while providing a fit indistinguishable from the more parsimonious model. For the sake of brevity, we will analyze the posterior only for this final model. 

% We model the reaction time data, then the percent correct. We predicted these variables based on \textsc{System status} (sham AI vs. no-AI) \textsc{System descrciption} and their interaction. 

%We can follow that the effect of \textsc{System Status} and \textsc{System description} on the TLX is negligible and not distinguishable from a null effect. \


%To replicate \citet{villa2023placebo}, we augmented post-interaction scales with the UEQ and applied a Bayesian between-subjects \textit{t}-test.

% To replicate \citet{villa2023placebo}, we have administered the same scales post-interaction augmented by the UEQ and tested them with a regression model resembling a Bayesian between-subjects \textit{t}-test with normal-distributed priors set for the intercept and the regression slopes at the item/scale mean with one standard deviation of the item/scale mean as standard deviation of the distribution. We found no differences whatsoever between the \textsc{System description} after the interaction, with the exception of the item "The AI system made the task easier" which was favorably answered for the positive verbal description, see \autoref{tab:customnscales}.
% We, therefore, further analyzed the rest of the items jointly and tested the items against an expected neutral value, i,e,., 4. Here, it only became apparent that participants slightly disagreed with the item "The task was easy" and did not agree with the control scale for an unspecific response "The AI system improved my cognitive abilities.". However, resembling \citet{kosch2022placebo,villa2023placebo}, participants agreed with the item "The AI system has a lot of potential for future development.". 
% Next, we analyzed UEQ scales as a function of \textsc{System Description} and tested them against a neutral value of zero. We found that participants rated the User experience overall positive and that there were no differences between group regarding hedonic or pragmatic attributes of the user experience as measured by the UEQ. 
% Then we inspected the overall usability as indicated by the System usability scale. Again we compared both \textsc{System Description} groups and also tested the value against the often proclaimed value of 68 being average usability. We found that the AI system was rated to have average usability and that \textsc{System Description} did not affect ratings in the System usability scale. 




% \begin{table}[tbh]
% \caption{Custom items were answered on a 7-point likert scale(1 - strongly disagree; 7 - strongly agree). We also report the SUS, the UEQ and the Trust-XXX. We compared the nocebo to the placebo group. Effects that are distinguishable from zero are marked with *.}
% \resizebox{\textwidth}{!}{  
% \begin{tabular}{lllllcl}
% \toprule
% Item/scale & $M_{nocecebo}$ (SD) & $M_{placebo}$ (SD) &  $M_{diff}$ & $\tilde{b}_\text{std}$ & $HDI_\text{95\%}$ &  $p_b$ \\
% \midrule
% \textit{The task was easy.}                             & 3.24 (1.62) & 3.65 (1.80) & -0.41 & 0.22 & {[}-0.26, 0.69{]} & 82.64\% \\
% \textit{The AI system made the task easier.}            & 3.36 (1.78) & 4.28 (1.48) & -0.92 & 0.50 & {[}0.03, 0.97{]} & 98.21\% \\
% \textit{The AI system made the task more enjoyable.}    & 3.33 (1.83) & 4.12 (1.49) & -0.79 & 0.40 & {[}-0.09, 0.89{]} & 95.20\% \\
% \textit{The AI system made me more self-confident.}     & 3.39 (1.49) & 4.06 (1.77) & -0.67 & 0.42 & {[}-0.04, 0.89{]} & 96.37\% \\
% \textit{The AI system made me more efficient.}          & 3.87 (1.55) & 4.25 (1.34) & -0.38 & 0.23 & {[}-0.25, 0.70{]} & 82.89\% \\
% \textit{The AI system improved my performance.}         & 3.96 (1.55) & 4.28 (1.39) & -0.32 & 0.17 & {[}-0.30, 0.64{]} & 77.58\% \\
% \textit{The AI system improved my cognitive abilities.} & 3.54 (1.39) & 4.28 (1.34) & -0.17 & 0.10 & {[}-0.37, 0.57{]} & 66.85\% \\ 
% \begin{tabular}[c]{@{}l@{}}\textit{The AI system has a lot of potential for future development.}\end{tabular} & 5.03 (1.15) & 5.46 (1.13) & -0.43 & 0.40 & {[}-0.08, 0.86{]} & 93.95\% \\ 
% System usability scale  & 64.62 (13.86) & 68.35 (17.50) & -3.73 & 0.21 & {[}0.33, 0.68{]} & 78.32\%\\
% UEQ-Pragmatic       & 0.53 (0.92) & 0.92 (1.22) & -0.39 & 0.36  & {[}-0.13, 0.79{]} & 92.97\%\\
% UEQ-Hedonic         & 0.73 (1.02) & 0.80 (1.29) & -0.07  & 0.05  & {[}-0.43, 0.53{]} & 57.93\%\\
% UEQ-Overall         & 0.63 (0.81) & 0.86 (1.13) & -0.23  & 0.21  & {[}-0.39, 0.76{]} & 78.94\%\\



% \bottomrule    
% \end{tabular}
% }
% \label{tab:customnscales}
% \end{table}

%To validate the previous observation that negative expectations about the AI system could not be induced, we conducted a separate online replication study. This replication study replicated the first part of the previous experiment but was concluded after assessing expectations and judgments of performance and tested the negative written narrative. We replaced the explanation of analyzing skin conductance levels the use of facial expressions derived from real-time video input in line with \citet{kosch2022placebo} (no camera stream was recorded). After reading the \textsc{system description}, participants were asked to complete a \textsc{comprehension check}. They were divided into two groups: the 51 participants of the first completed the check but received no feedback regarding the correctness of the answers. The second group consisted of 46 participants; they were required to repeat the check until all questions were answered correctly. The condition \textsc{comprehension check} was coded (no: -1/yes: 1). Comparisons were made on z-standardized data, and thus, regression weights depict deviation from the mean, similar to Cohen's D. After answering all questions, we asked participants to report why they chose these number of points with an open text field. 


% Regarding overall performance, participants showed a weaker agreement with performing better with the sham AI system after having to respond correctly to all the items in the comprehension check  ($M$ = 4.59, $SD$ = 0.963) than participants who could proceed without answering all items correctly ($M$ = 5.11, $SD$ = 1.12). This difference could be distinguished from zero $\tilde{b}_\text{comprehension check}$=  -0.26  [-0.47, -0.05] , $p_b$ = 0.77\%. However, overall performance in both groups remained very positive, \textsc{comprehension check} $\tilde{b}_\text{diff}$ = 0.52 [0.103 0.944], $p_b$ = 0.008\%, $p$ = 0.00\%. There was no indication in the posterior sample that either of the groups had negative expectations on performance with the AI active, which would be smaller than 4 on the Likert scale $\tilde{b}_\text{comprehension check: no}$=  0  [5.69  6.34], $p_b$ = 100\%, $\tilde{b}_\text{comprehension check: yes}$=  0  [5.16  5.77], $p_b$ = 100\%.

% For estimation of correct responses, we found a distinguishable main effect for $\tilde{b}_\text{system status}$ =  5.74  [2.16, 9.28], $p_b$ = 1.11\%%,  $\tilde{\delta}_\text{b}$ =  0.14 [0.05, 0.24]
% . We also found an interaction effect $\tilde{b}_\text{system status*comprehension check}$ =  5.74  [1.14, 8.28] , $p_b$ = 0.54\%%,  $\tilde{\delta}_\text{b}$ =  0.12 [0.03, 0.21]
% . When contrasting the estimated number of correct responses with and without the sham AI system active, the participants in the group without the enforced comprehension check estimated to answer more accurately with the sham AI system active ($M$ = 158.74, $SD$ = 33.34), than without ($M$ = 137.83, $SD$ = 42.37), $\tilde{diff}_\text{system status}$=  20.9 [10.6, 31.3], $p_b$ = <0.005\%.
% The group that had to answer all items in the comprehension check correctly did not differ in the estimated amount of correct responses between the \textsc{system status}\text{AI} ($M$ = 146, $SD$ = 42.3) or \textsc{system status}\text{no AI} ($M$ = 144, $SD$ = 38.3), \textsc{system status} $\tilde{b}_\text{diff}$ = 2.04 [-7.81, 11.9], $p_b$ = 33.9\%, but remained positive in both conditions with posterior samples indicating a negative difference (i.e. favoring no AI over AI) at $p$ = 0.01\%.
% The main effect for the enforced comprehension check between the groups could not be distinguished from 0 $\tilde{b}_\text{comprehension check}$ =  1.75  [-5.28,   8.89], $p_b$ = 31.36\%.

% A regression model was computed to assess the expected task speed of the participants with and without the sham AI system active with \textsc{comprehension check} as a predictor and an intercept of 50. The group with the forced comprehension check thought that they would be slower ($M$ = 61.45, $SD$ = 17.71) than the group that did not have to answer all items correctly ($M$ = 69.48, $SD$ = 19.47), $\tilde{b}_\text{comprehension check}$ = -4.02 [-7.73, -0.28], $p_b$ = 1.71\%. Nevertheless, there was no indication in the posterior sample that either of the groups had negative expectations on being slower (< 50) with the AI than without the AI on a scale from 0 (slower) to 100 (faster) $\tilde{b}_\text{comprehension check: no}$=  0  [14.1, 24.9], $p_b$ = 100\%, $\tilde{b}_\text{comprehension check: yes}$=  0  [6.22  16.5], $p_b$ = 100\%.
% However, both groups showed a positive  $\tilde{b}_\text{diff}$ = 8.04 [0.535  15.4], $p_b$ = 0.02\%.

%Across all quantitative measures of expectations, we find a common pattern. A comprehension check that enforced picking up the attribute could lower expectations with regard to overall performance, expected correct trials or task speed but even this strong manipulation could not turn positive expectations negative. We, thus, consider the finding that negative descriptions of an AI system cannot induce negative expectations with regard to performance to be replicable and robust. 


%This could be connected to the widespread emergence of new AI technologies that have improved participants' performance, such as large language models \steeven{cite something here and also fiona's preprint} and the increased accessibility of these AI models to the general public. In fact, by examining the potential for a nocebo effect at a different point in time, after the peak of excitement surrounding these technologies has subsided, it may be feasible to effectively induce a nocebo effect in individuals.

% \subsection{Robustness to Negative Verbal Descriptions}

% Our study reveals that the nocebo effect in Human-AI interaction does not follow the expected pattern of being proportionally negative to the placebo effect, challenging recent research on AI interaction expectations. Contrary to our initial hypothesis, individuals did not reduce their expectations based on the system description. This surprising resilience suggests that people's expectations of AI benefits remain robust even in the face of negative narratives (nocebo effect). This finding holds significance in the context of understanding how the interaction with these technologies influences user behavior and underscores the strength of the prevailing positive views about AI among the general population.

% In light of these findings, a central question arises: How does the nocebo effect impact various demographics, considering disparities in technology access, cultural influences, and their effects on AI perceptions? Recent research has shown that among technologies designed to enhance human performance, those related to cognitive augmentation, such as AI, tend to elicit more caution from individuals. Furthermore, both our study and related research on user expectations regarding AI often focus on initial interactions with the supporting system. This initial interaction might differ significantly from expectations after sustained use, and surprisingly, this aspect has received limited attention in the literature. Future research could explore the evolution of expectations in this context, shedding light on the dynamic nature of user perceptions of AI.
% In order to validate the robustness of AI to the nocebo effect, an effort in answering those questions must be made.

%Third, from a design perspective, our re
% Third, from a design perspective, the mere belief in AI assistance enhances user experience and performance. Emphasizing a system's "smart" capabilities is beneficial. However, balanced expectations in the human-centered design evaluation process are crucial to avoid the potential pitfalls of both placebo and nocebo effects.
% Fourth, societally, it is vital to meticulously assess technologies pre-market, especially those intended for critical applications. Implementing placebo controls is essential to ensure that both user experience and real-world utility are comprehensively evaluated, especially in technologies that have the potential to be used in critical settings like medical contexts.
%Third, in human-centered design,  where systems are typically compared based on user interaction, a placebo effect could lead to misinterpretation of results.   %Conversely, negative expectations (i.e., nocebo) could result in unnecessary or even harmful modifications to the AI system as a reaction to negative user feedback. 
 

% \subsection{Implications}
% We will use the implications in therk of \cite{} to structure the implications of our work. 

% \subsubsection{Methodological implications}

% While AI systems themselves appear to be resilient to the nocebo effect, we advise designers to steer clear of overly negative narratives when describing their systems or alternative systems (like the baseline). It's important to note that we found a resilience to the nocebo effect specifically for AI systems. We recommend further testing to determine if non-hyped systems also exhibit this level of resilience to negative narratives.



% %methodological implication: https://nielsvanberkel.com/files/publications/interactions2023a.pdf
% \subsubsection{Implications for the HCI community}

% We suggest that the HCI community consider the potential placebo and nocebo effects that technology narratives can have on users. Acknowledging these effects, whether influenced by popular or designer narratives, is essential for steering the field toward genuine innovation and insights. It's worth noting that these effects often go unnoticed by users, designers, or experimenters. By being mindful of these dynamics, we can promote more informed and effective developments in human-computer interaction.

% \subsubsection{Implications for design}

% It appears that just the belief in having an AI system assist with a task is sufficient to make users more at ease with the system, and it can even enhance certain performance aspects (such as accuracy in Kosch's study and reaction times in our current study). In an ideal scenario, designers would integrate a smart system to aid users. However, when that's not feasible, it would be advantageous to shape the narrative to emphasize any "smart" elements that the system might have. On the other hand, placebo effects could lead to adopting systems that bring no real benefits \cite{kosch2022placebo}, nocebo effects, on the other side, could make technology adaptation unreasonably conservative and stall innovation.  Only near-neutral expectations, if possible to implement, are desirable for evaluation in the HCD process.  
% %HCD process is messed up

% \subsubsection{Implications for practice}


% To navigate expectations in HCD appropriately, it's crucial to understand the role of negative and positive user expectations for technology evaluation.  For AI technology we find for now that AI's placebo is robust to negative verbal description and that even with large effort expectancy of performance cannot be turned negative but merely be decreased. 
% % product development needs placebo control --there is no way around it
% \subsubsection{Implications for society}
% % people should be cautious,
% At the societal level, there needs to be a distinct separation in how technologies are assessed before they enter the market. This differentiation is essential because many individuals make purchasing decisions not just based on the user experience a product offers, but also on the expected benefits it can provide.

% Hence, the implementation of placebo controls becomes particularly crucial, especially in technologies that have the potential to be used in critical settings like medical centers or emergency response systems. These controls help ensure that the evaluation of a technology takes into account not only the user experience but also the real-world impact and benefits it can deliver in practical and vital scenarios.
%Such a replication would help to shed light on the question of, Is the general narrative surrounding a technology or whether the technology in itself is insensitive to negative verbal descriptions.

%they can be estimated quite efficiently \cite{Voss_2015_ddm_cognitiveprocesses}, .... %.....AI systems exhibit resilience to the nocebo effect. Designers should avoid negative narratives, and additional investigations into non-hyped systems are warranted. %Reference: \href{https://nielsvanberkel.com/files/publications/interactions2023a.pdf}{source}.

%This could be linked to \citet{villa2023placebo} findings, where individuals perceive less self-relevance in decision-making when there's joint responsibility between the AI system and the human. This could have led to quicker decisions compared to situations where the individual bears full responsibility for the outcome. Further research in this area could provide insights into how AI affects the sense of agency in the context of Human-AI interaction.
